A Light Field Front-end for Robust SLAM in Dynamic Environments

There is a general expectation that robots should operate in urban environments often consisting of potentially dynamic entities including people, furniture and automobiles. Dynamic objects pose challenges to visual SLAM algorithms by introducing errors into the front-end. This paper presents a Light Field SLAM front-end which is robust to dynamic environments. A Light Field captures a bundle of light rays emerging from a single point in space, allowing us to see through dynamic objects occluding the static background via Synthetic Aperture Imaging(SAI). We detect apriori dynamic objects using semantic segmentation and perform semantic guided SAI on the Light Field acquired from a linear camera array. We simultaneously estimate both the depth map and the refocused image of the static background in a single step eliminating the need for static scene initialization. The GPU implementation of the algorithm facilitates running at close to real time speeds of 4 fps. We demonstrate that our method results in improved robustness and accuracy of pose estimation in dynamic environments by comparing it with state of the art SLAM algorithms.

==> sections/subsections/implementation.tex <==
\subsection{Implementation details}
The light field front-end is built on ORBSLAM2 as the base SLAM system. Even though we have restricted the classes of dynamic objects to just people to detect and generate pixel wise labels indicating dynamic and static content, our method is applicable to any moving or potentially movable objects if given an appropriate segmentation. We implemented maskRCNN\cite{he2017mask}and bodypix\cite{bodypix} or segmentation. The former is more accurate while the latter is faster. The depth map and refocused image of the static background are computed in a reference view. Without loss of generality we consider the leftmost image $X^1$ as the reference image.

During the energy minimization step we work in generalized disparity space to facilitate discrete optimization. We have an array of cameras where a unit shift in disparity between reference view may result in fractional shift with respect to another camera. Thus, while considering disparities for optimizing the energy function we make sure to include non-integral disparity values to account for multi baseline properties. The algorithm is implemented using CUDA on a GPU where each pixel is independently processed for depth estimation and compute the refocused image.This results in a highly parallel real-time algorithm.



==> sections/subsections/segmentationupdate.tex <==
\subsection{Segmentation update (E-step)}
\begin{figure*}[tb]
\centering
\includegraphics[width=0.31\linewidth]{figures/seg_prior.png}
\includegraphics[width=0.31\linewidth]{figures/ref_view_seg.png}
\includegraphics[width=0.31\linewidth]{figures/seg_update_ref.png}
\caption{Segmentation map update. \textit{left}: The initial segmentation prior from Bodypix.  \textit{center}: Segmentation labels obtained by simple thresholding.  \textit{right}: Final updated segmentation map.}
\label{fig:seg_update}
\end{figure*}
% high-level idea of the E-step
Assuming the segmentation algorithms is (near-) perfect, the solution to the graphical model described above is relatively straight forward. Unfortunately this proves difficult for many real-world scenarios as mentioned earlier. Modelling the segmentation as a hidden variable and the segmentation algorithm as a prior induces robustness, but comes at a cost of increased complexity of the E-step: the computation of the new segmentation distribution given the current estimate of disparity $\disparity^{old}$:

% E-step optimization problem
\begin{align}
p(\segmentation|\disparity^{old}, \pixels, \allPriors) &\propto p(\segmentation,\pixels|\disparity^{old},\allPriors)  \nonumber \\
&= \underbrace{p(x|\disparity^{old},\segmentation, \referencePixel)}_{\text{pixel likelihood}} \underbrace{\segmentationProbability}_{\segmentation\text{ prior}} \label{eq:e-step general}
\end{align}

% description E-step equation
The first term term, the pixel likelihood, has been discussed prior (in the M-step).
% shape of p(S)
The segmentation posterior is assumed to factorize into its independent pixels, $p(\segmentation) = \prod_k p(\segmentation^K)$, where $p(\segmentation^K)$ is modelled as a delta function (e.g. 'hard assignment'). It is feasible to enumerate over these, and hence the E-step results in finding the most likely assignment of $\segmentation$: the one that maximizes (where we have substituted~\cref{eq:e-step general} with their distributions): 

\begin{equation*}
    E(\segmentation) = \beta\; Var(f(x^1),...,f(x^k)) \segmentationProbability
\end{equation*}

This results in a more accurate estimation of segmentation, which in turn helps produce a better refocused image. The number of EM iterations depends on the initial quality of the segmentation algorithm.
